Emerging chromo-natural inflation

The shift-symmetric coupling of a pseudo-scalar particle driving inflation to gauge fields provides a unique way of probing cosmic inflation. We show for an SU(2) gauge group how a classical isotropic background gauge field develops from the standard quantum mechanical vacuum in the far past. Over the course of inflation, the theory dynamically evolves from an approximately abelian regime into an inherently non-abelian regime, with distinct predictions for the scalar and tensor power spectra. The latter regime closely resembles a setup known as chromo-natural inflation, although our main focus here is on a new part of the parameter space which has received little attention so far. For single-field slow roll inflation models, large scales may exit the horizon in the abelian regime, ensuring agreement with the observations of the anisotropies in the cosmic microwave background, whereas smaller scales experience the non-abelian effects. This results in a strong enhancement of the stochastic gravitational wave background at small scales, e.g. at frequencies accessible with ground-based interferometers. For the scalar power spectrum, a similar enhancement arises due to non-linear contributions.

==> GWs.tex <==
\section{Scalar and tensor power spectra}




Demonstrate how to compute the scalar and tensor power spectrum in the (N-A) regime. The problem is that we cannot relate this to observables, if the (V) regime is reached before the end of inflation, since then we don't know the overall e-fold we are at. Possible way out: choose parameters such that this regime is not reached before the end of inflation. \textit{Maybe better way out: in this section only, discuss SU(2)xU(1) model. I.e.\ the background evolution is as in standard abelian axion inflation (since we have demonstrated that the non-abelian contribution is subdominant for equal coupling), check here if there are relevant additional contributions to the power spectra (could be, due to linear contributions in stress-energy tensor).}
\begin{itemize}
\item scalar power spectrum: determined by $\delta \phi$ fluctuations computed above.
 \item Present general calculation of stochastic gravitational wave background produced from the enhanced gauge field modes.
 \item calculate stress energy tensor (see stress-energy tensor.pdf). 
 \item calculate tensor power spectrum. not linear contributions.
 \item equivalently: include eom for $\gamma_{ij}$ in coupled ODE system
 \item other pheno consequences?
\end{itemize}
